D-LoRa: a Distributed Parameter Adaptation Scheme for LoRa Network

The deployment of LoRa networks necessitates joint performance optimization, including packet delivery rate, energy efficiency, and throughput. Additionally, multiple LoRa parameters for packet transmission must be dynamically configured to tailor the performance metrics prioritization across varying channel environments. Because of the coupling relationship between LoRa parameters and metrics, existing works have opted to focus on certain parameters or specific metrics to circumvent the intricate coupling relationship, leading to limited adaptability. Therefore, we propose D-LoRa, a distributed parameter adaptation scheme, based on reinforcement learning towards network performance. We decompose the joint performance optimization problem into multiple independent Multi-Armed Bandit (MAB) problems with different reward functions. We have also built a comprehensive analytical model for the LoRa network that considers path loss, quasi-orthogonality of spreading factor, and packet collision. Experimental results show that our scheme can increase packet delivery rate by up to 28.8% and demonstrates superior adaptability across different performance metrics.

==> sections/11-motivation.tex <==
\section{motivation}
In the experiment shown in Fig. \ref{Fig1} and Fig. \ref{Fig2}, there are 50 nodes with stochastic data size\cite{mefi} in target area, whose size length is equal to 200m, and three energy-constrained UAVs which start from Charging Station (CS) CS0, CS2, and CS3 respectively. 
In the process of data collection, when the UAV energy is not enough to complete the task, the UAV would return to the CSs to charge itself\cite{hdrl}.
Try to use ACO in stochastic environment to iteratively derive an effective and versatile pheromone matrix, aiming to determine the paths for UAVs, and test the matrix in a fixed environment. 
However, from the metric of the data collection task completion time, the iterative matrix does not converge in the end, and the performance gradually deteriorates due to the influence of stochastic environment.
The collect data time of the same node varies with the environment, resulting in the instability of matrix update.

\begin{figure}[t]
\centerline{\includegraphics[width=0.4\textwidth]{fig/topo161717.png}}
\caption{The Location of ACO Algorithm Simulation}
\label{Fig1}
\end{figure}
\begin{figure}[t]
\centerline{\includegraphics[width=0.42\textwidth]{fig/antFinishTime2.png}}
\caption{The Completion Time of ACO Algorithm}
\label{Fig2}
\end{figure}
